A Time-Dependent TSP Formulation for the Design of an Active Debris Removal Mission using Simulated Annealing

This paper proposes a formulation of the Active Debris Removal (ADR) Mission Design problem as a modified Time-Dependent Traveling Salesman Problem (TDTSP). The TDTSP is a well-known combinatorial optimization problem, whose solution is the cheapest mono-cyclic tour connecting a number of non-stationary cities in a map. The problem is tackled with an optimization procedure based on Simulated Annealing, that efficiently exploits a natural encoding and a careful choice of mutation operators. The developed algorithm is used to simultaneously optimize the targets sequence and the rendezvous epochs of an impulsive ADR mission. Numerical results are presented for sets comprising up to 20 targets.

==> GAsection.tex <==
\section{Genetic Algorithm}\label{sez:GA}
%With a slight abuse of nomenclature,  terms \textit{individual} and \textit{chromosome} will be used alternatively	to denote a solution. 


A Genetic Algorithm (GA) is used in the present paper for solving the combinatorial optimization problems described in the previous sections.
%
%In the present paper, the solution of the combinatorial optimization problems defined in Sections~\ref{sez:timeUniformTour}-\ref{sez:timeDiscreteTour} will be searched for by using a Genetic Algorithm (GA).
Genetic algorithms  are well-known   population-based meta-heuristic  techniques inspired by natural evolution.
They have been successfully applied to a wide range of real-world problems of significant complexity. 
A brief overview of the algorithm is here presented. Interested readers are suggested to refer to Reference~\citenum{Mitchell1998} for further details.
%
A  block diagram of the basic algorithm is proposed in Figure~\ref{fig:GAflow}, 
highlighting  the presence of  three fundamental genetic operators (selection, crossover, and mutation)
which form the backbone of any GA implementation.

%\begin{figure} 
%\centerline{\includegraphics[width=0.25\columnwidth%]{Figures/GAflow2.jpg}}%
%\caption{GA flowchart}
%\label{fig:GAflow}
%\end{figure}

 \begin{minipage}{.41\linewidth}
\centering
\includegraphics[width=0.45\columnwidth]{Figures/GAflow2.jpg}
\captionof{figure}{Flow chart of Genetic Algorithm}
\label{fig:GAflow}
  \end{minipage}
\begin{minipage}{.47\linewidth}
\centering
        \begin{algorithm}[H]\small
        \caption{PMX}
        \begin{algorithmic}
 	\State Choose two random index $a$, $b$ so that   $0 \le a<b \le L$
 	\ForAll{ $i \in [a,b]$} 
 		\State $o_1[i] \gets p_2[i]$
 	\EndFor
 	\State $c \gets p_2[a:b]$ 
 	\ForAll{ $i \in \left[1, a-1] \cup [b+1,N\right] $ }  
 		\State $J\gets p_1[i]$ \Comment Proposal
 		\While { $J  \in c$}
 	
	 		\State  find iJ so that $p_2[iJ] == J$ \Comment  map $p_1$ into $p_2$
	 		\State  $J\gets p_1[iJ]$ \Comment New proposal
 		\EndWhile
 	 	\State $o_1[i] \gets J$ \Comment Accept the proposal
 	\EndFor 
\end{algorithmic}
\end{algorithm}
\captionof{figure}{Partially Mapped Crossover algorithm}
\label{alg:PMX}
\end{minipage}
\medskip

At the beginning, 	
an initial \textit{population}, that is, a collection of solutions (often referred as \textit{individuals} or \textit{chromosomes}) is randomly generated, with an attempt to cover the search space as best as possible. 
%
At each iteration (i.e.,  \textit{generation}), 
the fitness of each individual in the population is  evaluated first.
% SELECTION
Then, a mating population is created by selecting a number of individuals from the current population, according to a  \textit{selection operator}, 
which tries to promote individuals with a good fitness, without sacrificing diversity too much.
%
%One should avoid to make the population collapsing over a single individual.
Typical selection operators are Stochastic  Roulette Wheel and Tournament,\cite{Mitchell1998}
the latter  being the one used in the present application.
%
% CROSSOVER 
%
Next, %a new population is created from the mating population: 
pairs of individuals (parents) are  randomly chosen from the mating population and combined for producing new solutions (offsprings) according to a \textit{crossover}  rule. 
The underlying idea is that combining good solutions in some way allows to create new, and  hopefully better, solutions.
The process is repeated until a new population (usually with the same dimension of the previous one) is created.
%
% Mutation 
%
Eventually, a few randomly-chosen individuals of the offspring population undergo a mutation process, with the aim of increasing the population diversity.
%mutation rule and rate of mutation vary according to the specific mutation operator implemented in the code.
%
This new population eventually replaces the previous one and the process is repeated until some termination criterion (e.g., maximum number of generation) has been met.
%
%\hl{elitims}
As a minor, yet important, tweak,
\textit{Elitism} is enforced, that is, at the end of each generation, the $N_p^e$ best individuals of the parent population are copied into the offspring population, thus preserving the best solution from being accidentally lost in the evolution process. 
%
%\hl{epidemia - Diversity control}\\
Some control over the population diversity is often needed. The aim is to avoid an excessive uniformity between individuals that would result in a very inefficient use of the crossover operator, hence in a waste of function evaluations.
To overcome this problem, an \textit{epidemic} mechanism is introduced.
A diversity metric is defined as the sum over the population of the infinity-norm between any pair of individuals in the search space.
If the diversity score falls below a given threshold, a large part of the population dies, that is, it is randomly re-initialized.
This mechanism cannot happens more than $N^{epidemic}$ times and not two times within a number $N_G^{epidemic}$ of generations.  
%\hl{TODO}
 
%\hl{
%Of course, one can code an integer as a bit string but for sequencing and scheduling
%problems often other codes are used. For permutation problems, where the set of solutions
%is characterized by the set of all (or a subset of all) permutations of n jobs often the job or
%permutation code is used. An individual (solution) is described by a job sequence, and the
%i-th gene contains the index of the job on position i.
%However, when applying a classical crossover operator to individuals described in a
%permutation code, the offspring are often infeasible. There have been developed several
%operators that repair illegal offspring so that all offspring describe feasible individuals. The
%most popular and standard crossover operators are the PMX, the OX, the LOX, the CX
%operator, the OBX operator and the PBX operator. Most of these operators are two-point
%crossovers. We describe them in the terminology of the job code and generate one offspring}
%\midskip


 
While selection operators are usually problem-independent, 
crossover and mutation operators are tightly related to the adopted \textit{encoding}, that is, 
the way the real-word problem is described in terms of numerical variables.
Depending on the features of the decision variables, 
several encodings have been defined, with the most common being 
 binary, integer-valued, and real-valued %and tree[X]
encoding. 
%
In order to match the formulation developed in Section \ref{sez:Tour},
a permutation encoding   is here considered, that is,
each \textit{individual} or \textit{chromosome} is a permutation $\bfp\in\mathcal{P}^L$.  
Each gene takes an integer value in the range $\left[1,\ldots, L \right]$,
and two genes in the same \textit{individual} can not have the same value at one time.
%
%\hlc[green]{The intuition suggests that the best results are attained by an encoding that is "as natural as possible" for the problem at hand.}
%
Standard, general-purpose, crossover operators (such as, one-point, two-point, or uniform crossover) cannot be applied to a permutation without producing unfeasible offspring, that is, introducing multiple copies of the ``entries''.
However,
several permutation-preserving genetic operators, which have been developed for the permutation encoding in the context of the TSP problem, can be employed for solving the problem under investigation,
such as Partially Matched Crossover, Cycle Crossover, Order  Crossover,  Non-Wrapping Order Crossover, as well as many others.\cite{cicirello2006gecco,umbarkar2015crossover}

% 
%Among these, the Non-Wrapping Order Crossover (NWOX) operator\cite{cicirello2006gecco}, which is a slight modification of the Order  Crossover (OX1) operator, has been chosen for the present investigation,   which retains retain the strong order based characteristic of OX, but also to respect the absolute positioning of the values within the parent permutations.  This operator has been designed in the contest of scheduling problems where  the order of jobs in the sequence is highly important to the fitness of the solutions, but for which absolute position is also important to an extent.

The Partially Matched Crossover (PMX) devised by Goldberg\cite{goldberg1985alleles} has been adopted in the present paper,
as it aims to preserve both the order and position of as many entries as possible from the parents.
A Pseudo-code of this algorithm is presented in Figure~\ref{alg:PMX}.
An offspring is created starting from a sub-string (or \textit{cut}) of the first parent ($p_1$), in the same fashion as in a two-point crossover.
The remaining entries are taken from the other parent ($p_2$).
Entries not appearing in the cut are kept in the same position as they appear in $p_2$. Conflicts are resolving using $p_1$ as a map for $p_2$.

 %\hlc[green]{da cambiare}\hl{
%The order based crossover operator selects at random several
%positions in one of the parent tours, and the order of the cities in
%the selected positions of this parent is imposed on the other
%parent to produce one child. The other child is generated in an
%analogous manner for the other parent 
%}

Mutation operators are also of great relevance in the framework of genetic algorithms,  
% of combinatorial optimization problems 
as they allow to escape from situations of premature stagnation of the population on a sub-optimal solution,
and their impact on the effectiveness of the algorithm should not be underestimated.
Once again, an abundance of permutation-preserving mutation operators are documented in literature. % in the contest of the TSP and other combinatorial optimization problems. 
%
% [Safeguard] 
%three mutation operators, namely swap, insert, and reverse were adopted. Each time a mutation is called, one of the operators is randomly chosen and applied to the specified individual .
In the present application, a reverse mutation operator is adopted:
whenever an individual $\bfp$ must be mutated, 
two indices $i<j$ are randomly chosen and the new individual $\bfp^{new}$ is created as a copy of the original one, but for the genes from $i$ to $j$ that are copied in a reversed order, that is $\bfp^{new}(i:j) = \bfp(j:i)$.


%\begin{center}
%	\hl{descrizione degli operatori di mutazione}
%\end{center}
%two random index $r_1 <  r_2$ are chosen and the new chromosome $x^{new}$ is created from the original one $x$ accoriding to the rule
%$x^{new}(r_1:r_2) = x^{new}(r_2:r_1) $
%\hl{Maximum distance between the two random indexes can be bounded, reducing the occurrence of excessively-disruptive mutations.
%}
%$d_{max} = max\left\{ 3,\, D/7 \right\}$ has been chosen according to experience.






\subsection{GA hyperparameter}


The performance of a genetic algorithm clearly depends on 
the choice of selection,  mutation  and crossover operators,
%
but also on several ``hyper-parameters'', such as  
population size ($n_P$), 
number of generations ($n_G$), 
%crossover operator ($\star X$) and
crossover probability ($p_c$), that represents the percentage of the parents replaced by offspring,
%mutation operator ($\star M$) and 
mutation rate ($p_m$),
that is, the probability that one individual will undergo a random mutation,
%
and other operator-specific parameters, such as the depth of the reverse operator (i.e., the maximum number of element of the swath that will be reversed).
%
A proper tuning of these hyperparameters may greatly improve the solution capability of GA.
However, the optimal tuning of a genetic algorithm  is documented to be problem dependent, and represents an NP-hard problem by itself.
Therefore, a preliminary tuning is usually done on a simplified, possibly scaled, version of the optimization problem of interest,
with the hope to capture all the relevant features of the original problem.






 
%   
%Algoritmo 1
%\begin{enumerate}
%\item permutation encoding
%\item O1X crossover
%\item reverse mutation 
%\end{enumerate}
%
%  




==> Solutions/Compare8.tex <==
\begin{tabular}{l c c c } 
\hline \hline
& \textbf{SA} & \textbf{DE} & \textbf{DE} \\ 
& & time-fixed & time-free \\ 
\hline 
\textbf{8x1}: $\Delta v_{tot} = \, \SI{}{\kilo\m}/\SI{}{\s}$ & 0.5061 & 0.4931 & 0.4408 \\ 
\textbf{8x2}: $\Delta v_{tot} = \, \SI{}{\kilo\m}/\SI{}{\s}$ & 0.3767 & 0.3722 & 0.3587 \\ 
\textbf{8x3}: $\Delta v_{tot} = \, \SI{}{\kilo\m}/\SI{}{\s}$ & 0.3344 & 0.3296 & 0.2969 \\ 
% \textbf{8x4}: $\Delta v_{tot} = \, \SI{}{\kilo\m}/\SI{}{\s}$ & 0.3164 & 0.3127 & 0.2973 \\ 
\hline \hline
\end{tabular} 


==> Solutions/Solution8.tex <==
\begin{tabular}{l c c c c c c c c } 
\hline \hline
\multicolumn{9}{c}{\textbf{Mission 8x1:} $\Delta v_{tot} = 0.44092\, \SI{}{\kilo\m}/\SI{}{\s}$} \\ 
\hline 
ID & 8 & 6 & 7 & 5 & 4 & 3 & 2 & 1 \\ 
$t\, [\SI{}{\day}]$ & 0.5050 & 1.0851 & 1.5569 & 1.8889 & 2.4740 & 2.6984 & 3.3499 & 3.7777 \\ 
$\Delta v\, [\SI{}{\kilo\m}/\SI{}{\s}]$ & 0.0340 & 0.0270 & 0.0109 & 0.0163 & 0.1450 & 0.0481 & 0.0951 & 0.0644 \\ 
%$N_{\Delta v}$ & 4 & 2 & 2 & 2 & 3 & 4 & 3 & 4 \\ 
\hline 
\hline 
\multicolumn{9}{c}{\textbf{Mission 8x2:} $\Delta v_{tot} = 0.35851\, \SI{}{\kilo\m}/\SI{}{\s}$} \\ 
\hline 
ID & 6 & 8 & 5 & 7 & 4 & 3 & 2 & 1 \\ 
$t\, [\SI{}{\day}]$ & 0.2830 & 0.5894 & 0.7794 & 1.1100 & 1.6894 & 1.9526 & 2.8445 & 3.7777 \\ 
$\Delta v\, [\SI{}{\kilo\m}/\SI{}{\s}]$ & 0.0217 & 0.0270 & 0.0324 & 0.0644 & 0.1275 & 0.0054 & 0.0556 & 0.0244 \\ 
%$N_{\Delta v}$ & 2 & 2 & 2 & 3 & 3 & 2 & 4 & 3 \\ 
\hline 
\hline 
\multicolumn{9}{c}{\textbf{Mission 8x3:} $\Delta v_{tot} = 0.29694\, \SI{}{\kilo\m}/\SI{}{\s}$} \\ 
\hline 
ID & 1 & 3 & 2 & 4 & 7 & 5 & 6 & 8 \\ 
$t\, [\SI{}{\day}]$ & 0.0788 & 0.4176 & 0.6928 & 0.7870 & 1.5407 & 1.6361 & 1.7625 & 3.7777 \\ 
$\Delta v\, [\SI{}{\kilo\m}/\SI{}{\s}]$ & 0.0545 & 0.0325 & 0.0294 & 0.0165 & 0.0808 & 0.0163 & 0.0054 & 0.0616 \\ 
%$N_{\Delta v}$ & 2 & 3 & 3 & 2 & 3 & 2 & 2 & 3 \\ 
\hline 
%\hline 
%\multicolumn{9}{c}{\textbf{Mission 8x4:} $\Delta v_{tot} = 0.29739\, \SI{}{\kilo\m}/\SI{}{\s}$} \\ 
%\hline 
%ID & 1 & 3 & 2 & 4 & 7 & 5 & 6 & 8 \\ 
%$t\, [\SI{}{\day}]$ & 0.0998 & 0.3756 & 0.6375 & 0.7260 & 1.5322 & 1.6993 & 1.7680 & 3.7777 \\ 
%$\Delta v\, [\SI{}{\kilo\m}/\SI{}{\s}]$ & 0.0545 & 0.0417 & 0.0263 & 0.0165 & 0.0750 & 0.0163 & 0.0054 & 0.0617 \\ 
%$N_{\Delta v}$ & 2 & 3 & 4 & 2 & 3 & 2 & 2 & 3 \\ 
\hline 
\end{tabular} 


==> TSP.tex <==
\newcommand{\mysum}[3]{\sum_{#1 = #2}^{#3}}

In this Section, the Traveling Salesman Problem (TSP) and its Time-Dependent variants are presented and formulated both as Integer Linear Programming (ILP) problems and as Permutation Optimization (PO) problems.

\subsection{TSP}
The original Traveling Salesman Problem deals with the determination of a minimum-distance tour
for a salesman that, departing from his home city, has to visit exactly once each city on a given list, and then come back home \cite{lawler1985traveling}.
The TSP is one of the most studied combinatorial optimization problems; nevertheless, no resolving algorithm with polynomial-time complexity has been found so far.

The TSP is often formulated as an ILP.
Let $x_{ij}$ be a binary variable indicating whether or not the salesman goes directly from city $i$ to city $j$:
\begin{equation}
	x_{ij} = \begin{cases}
	1 & \text{if the salesman goes from city $i$ to city $j$} \\
	0 & \text{otherwise}
	\end{cases}
\end{equation}

Denoting the cost of going from city $i$ to city $j$ by $c_{ij}$, the TSP is solved by the matrix $X = (x_{ij})$ which minimizes the tour cost:
\begin{equation}
	\mysum{i}{1}{n} \mysum{j}{1}{n} c_{ij} x_{ij}
	\label{eq:TSP_cost}
\end{equation}
where $n$ is the total number of cities, i.e. the cardinality of the cities set $V = \{1, \dots, n\}$.

Meanwhile, the following constraints must be satisfied:
\begin{align}
	\mysum{j}{1}{n} x_{ij} &= 1 \text{, } \hspace{10mm} i = 1, \dots, n \label{eq:each_row_con} \\
	\mysum{i}{1}{n} x_{ij} &= 1 \text{, } \hspace{10mm} j = 1, \dots, n \label{eq:each_col_con}
\end{align}
where the constraint \eqref{eq:each_row_con} (respectively, \eqref{eq:each_col_con}) ensures that the salesman departs (respectively, arrives) once from (respectively, in) each city. 

Actually, Eqs.~\ref{eq:TSP_cost} to \ref{eq:each_col_con} describe the \textit{assignment problem}, a well known P-complexity problem. However, a solution to the assignment problem could be a set of disconnected \textit{subtours}, i.e., closed loops of a subset $S \subset V$ with $|S| < n$ cities.

So, in order to prevent subtours (that are not allowed in the TSP), $2^n - 2$ additional constraint must be added \cite{dantzig1954solution}:
\begin{equation}
	\sum_{i \in S} \sum_{j \in S} x_{ij} \leq |S| - 1, 
\end{equation}
The need for blocking subtours makes the TSP an NP-hard problem.
So, overall, $n^2$ binary variables have to be determined, subjected to $2^n + 2n - 2$ linear constraints.


Although the ILP formulation of the TSP has found a considerable success in literature, the problem can be more easily (and naturally) formulated also as a Permutation Optimization problem: the goal is to find the shortest Hamiltonian cycle of $n$ cities, i.e. a cyclic permutation $\pi$ of the numbers $\{1, \dots,  n\}$ which minimizes: 
\begin{equation}
	\mysum{i}{1}{n-1} c_{\pi(i) \pi(i+1)}
	\label{eq:TSP_cost}
\end{equation}
where $C = (c_{ij})$ is a $n \times n$ distance matrix.
It is evident that, with respect to the ILP formulation, only $n$ (integer) variables made up the solution vector.

One final, but important, remark on the TSP. If the initial city has to be a pre-assigned one $s$ (as in the ADR mission design problem here considered), it is sufficient to set null the cost of arriving to $s$. So the $s$-th column of the distance matrix $c_{ij}$ has to be set to zero. In this way, a ``closed'' TSP problem can be still solved, but since the cost of the transfer from the "final" city to the pre-assigned initial one is null, it does not affect the objective function. 

\subsection{The Time-Dependent TSP}
In the The Time-Dependent variant of the TSP, the distance matrix $C$ changes according to the time the cities are visited.
The different formulations of the problem reported in literature can be substantially traced back to two basic cases, of increasing complexity \cite{Bentner2001}.

\subsubsection{Approach A}
In a first formulation of the TDTSP, the cost of each transfer depends only on the position that the transfer occupies in the whole tour. This problem can be formulated as an ILP problem by introducing 
$n$ time periods, indexed by $t$, and a time-variant distance tensor $C =( c_{ijt})$, where $c_{ijt}$ indicates the cost of going directly from city $i$ to $j$ at time $t$.
Variables $x_{ijt}$ are correspondingly defined.
The objective function to be minimized is now:
\begin{equation}
	\mysum{i}{1}{n}\mysum{j}{1}{n}\mysum{t}{1}{n} c_{ijt} x_{ijt}
\end{equation}

Assuming a tour that begins and ends in city 1, the constraints are:
\begin{align}
	\mysum{j}{1}{n} \mysum{t}{1}{n} x_{ijt} &= 1 \text{, } \hspace{10mm} i = 1, \dots, n \label{eq:each_row_con_tdtsp} \\
	\mysum{i}{1}{n} \mysum{t}{1}{n} x_{ijt} &= 1 \text{, } \hspace{10mm} j = 1, \dots, n \label{eq:each_col_con_tdtsp} \\
	\mysum{i}{1}{n} \mysum{j}{1}{n} x_{ijt} &= 1 \text{, } \hspace{10mm} t = 1, \dots, n \label{eq:each_time_con_tdtsp} \\
	\mysum{j}{1}{n} \mysum{t}{2}{n} t x_{ijt} - \mysum{j}{1}{n} \mysum{t}{1}{n} t x_{jit} &= 1 \text{, } \hspace{10mm} i = 2, \dots, n \label{eq:flux_con_tdtsp}
\end{align}
Constraints \ref{eq:each_row_con_tdtsp} to \ref{eq:each_col_con_tdtsp} ensure that exactly one transfer is performed from and to each city, while constraint \eqref{eq:each_time_con_tdtsp} ensures that each transfer takes place at a different time period.
Instead, Eq. \eqref{eq:flux_con_tdtsp} guarantees that the difference between the departure time and the arrival time is unitary.

This formulation contains $n^3$ variables and $4n - 1$ constraints. The number of constraints can be further reduced to n by replacing Eqs.~\ref{eq:each_row_con_tdtsp} to \ref{eq:each_time_con_tdtsp} with the only constraint\cite{gavish1978travelling}:
\begin{equation}
	\mysum{i}{1}{n}\mysum{j}{1}{n}\mysum{t}{1}{n} x_{ijt} = n
	\label{eq:total_transfers_tdtsp}
\end{equation}

However, in order to force the tour to begin and end at vertex 1, some of the objective coefficients must be set to infinity or zero:
\hl{la descrizione che segue puo' essere rimossa se abbiamo problemi di spazio, tenendoci sul generico, e magari rimandando alla fonte e fine}

\hl{DA QUI}
\begin{align}
	c_{i1t} &= \infty \text{, } \hspace{10mm} i = 1, \dots, n \text{, } t = 1, \dots, n - 1 \label{eq:con_forbid_intemediate_return} \\
	c_{i1n} &= 0 \text{, } \hspace{10mm} i = 1, \dots, n \label{eq:con_cost_free_return} \\
	c_{1jt} &= \infty \text{, } \hspace{10mm} j = 2, \dots, n \text{, } t = 2, \dots, n \label{eq:con_forbid_intemediate_departure} \\
	c_{ij1} &= \infty \text{, } \hspace{10mm} i = 2, \dots, n \text{, } j = 2, \dots, n \label{eq:con_forbid_other_initial_transfers} \\
	c_{ijn} &= \infty \text{, } \hspace{10mm} i = 2, \dots, n \text{, } j = 2, \dots, n \label{eq:con_forbid_other_final_transfers}
\end{align}
Constraints \eqref{eq:con_forbid_intemediate_return} and \eqref{eq:con_cost_free_return} forbid any transfer to return to the initial city, except for the last one ($t = n$), that is cost-free since we are solving an Hamiltonian path problem.
Instead, the constraint \eqref{eq:con_forbid_intemediate_departure} forbids departure from the chaser at times different than the initial one.
On the other hand, the constraints \eqref{eq:con_forbid_other_initial_transfers} and \eqref{eq:con_forbid_other_final_transfers} forbid any transfer not involving city 1 respectively at the initial and final period.

\hl{A QUI}

The formulation of the present TDTSP as a PO problem is far easier to devise. 
The objective is to determine the permutation $\pi$ of the numbers $\{1,\dots,n\}$ which minimizes:
\begin{equation}
	\mysum{i}{1}{n-1} c_{\pi(i) \pi(i+1) i}
	\label{eq:TSP_cost}
\end{equation}
where the distance tensor $C = (c_{ijt})$ is the same as before.
Although $n$ time periods have been introduced, the number of variables is still $n$. \hl{questo evidenzia come sia migliore la formulazione a permutazione}

\subsubsection{\hl{Approach B}}
In the previous formulation all the departures and arrivals had to take place at the time nodes.
In a second, more general, formulation, the cost of each transfer depends both on the starting time and on the duration of the transfer itself.
This problem corresponds to a TDTSP where there are more time periods (at limit infinite) than cities and only at some of these times a transfer actually takes place. 

Let us consider $n_t$ time periods, indexed by $t$, and a distance tensor $C = (c_{ijtm})$, where $c_{ijtm}$ is the cost of departing from city $i$ at time $t$ and arrive at city $j$ at time $t + m$. 
Again, variables $x_{ijtm}$ are correspondingly defined.
The objective function to be minimized is now:
\begin{equation}
    \mysum{i}{1}{n}\mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} c_{ijtm} x_{ijtm}
\end{equation}
$M$ is the maximum duration of a transfer. It can be determined a priori as $M = n_t - (n - 1)$.

This problem is a generalization of the previous one: indeed, if all transfers last the same amount of time, the previous formulation (Approach A) is obtained. 
Hence the constraint structure is quite similar.
The total number of transfers must be $n$, so the constraint \eqref{eq:total_transfers_tdtsp} becomes:
\begin{equation}
		\mysum{i}{1}{n}\mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} x_{ijtm} = n \label{eq:total_transfers_m_tdtsp} \\
\end{equation}

Differently from before, the constraint \eqref{eq:total_transfers_m_tdtsp} on this finer time mesh does not guarantee that all cities are visited.
In order to include each city in the tour, one departure and one arrival must be ensured for each one, thus the constraints \eqref{eq:each_row_con_tdtsp} and \eqref{eq:each_col_con_tdtsp} become:
\begin{align}
	\mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} x_{ijtm}  &= 1 \text{, } \hspace{10mm} i = 1, \dots, n \label{eq:each_row_con_m_tdtsp} \\
	\mysum{i}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} x_{ijtm}  &= 1 \text{, } \hspace{10mm} j = 1, \dots, n \label{eq:each_col_con_m_tdtsp}
\end{align}

The main difference from the previous formulation is the duration of each transfer. While before every transfer length was unitary, now it is of length $m$.
The generalization of the flux constraint \eqref{eq:flux_con_tdtsp} is:
\begin{equation}
	\mysum{j}{1}{n}\mysum{t}{2}{n_t}\mysum{m}{1}{M} t x_{ijtm} - \mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} t x_{jitm} = \mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} m x_{jitm} \text{, } \hspace{10mm} i = 2, \dots, n \label{eq:flux_con_m_tdtsp}
\end{equation}
Finally, in order to limit the total duration of all transfers inside the time grid, the following additional constraint must be ensured:
\begin{equation}
	\mysum{i}{1}{n}\mysum{j}{1}{n}\mysum{t}{1}{n_t}\mysum{m}{1}{M} m x_{ijtm} \leq n_t \label{eq:max_m_sum}
\end{equation}

Finally, assuming a tour that begins and ends at city 1, the objective coefficients are set as in Eqs. \ref{eq:con_forbid_intemediate_return} to \ref{eq:con_forbid_other_final_transfers}, except for \eqref{eq:con_forbid_intemediate_return} that becomes:
\begin{equation}
	c_{i1t} = \infty \text{, } \hspace{10mm} i = 1, \dots, n \text{, } t = 1, \dots, n_t - M \label{eq:con_forbid_intemediate_return_m}
\end{equation}


%	c_{i0n} &= 0 \text{, } \hspace{10mm} i = 1, \dots, n \\



\hlc[green]{LF} - 
scriverei qui sotto la formulazione su base permutazione per entrambi i casi, introducendo l'idea di permutazione aumentata dell'outer-level problem

==> Test.tex <==

\begin{table}[h!]
\centering
\begin{tabular}{ccccc}
$\bm{t\, [T_0]}$ & $\bm{\Delta \theta\, [deg]}$ & \begin{tabular}[c]{@{}c@{}}\textbf{Lambert}\\ $\bm{\Delta V\, [km/s]}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Heuristic}\\ $\bm{\Delta V\, [km/s]}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Optimal}\\ $\bm{\Delta V\, [km/s]}$\end{tabular} \\ \hline
& 45 & 5.1681 & 0.12472 & 0.12293 \\
 & 90 & 1.0927 & 0.33035 & 0.32798 \\
 & 135 & 0.9112 & 0.53032 & 0.52362 \\
 & 180 & 0.87041 & 0.72495 & 0.68931 \\
 & 225 & 2.1923 & 0.76225 & 0.63299 \\
 & 270 & 0.6971 & 0.52996 & 0.46291 \\
 & 315 & 0.70947 & 0.30502 & 0.28079 \\
\multirow{-8}{*}{3.5} & 360 & 0.59949 & 0.086939 & 0.085642 \\ \hline
 & 45 & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} \\
 & 90 & 1.0447 & 0.11502 & 0.11197 \\
 & 135 & 0.40023 & 0.2107 & 0.20355 \\
 & 180 & 1.011 & 0.30516 & 0.29844 \\
 & 225 & 2.0954 & 0.38297 & 0.37106 \\
 & 270 & 1.6394 & 0.28063 & 0.27904 \\
 & 315 & 0.50717 & 0.1797 & 0.17961 \\
\multirow{-8}{*}{7} & 360 & 0.23748 & 0.080146 & 0.079859  \\ \hline
& 45 & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} \\
 & 90 & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} & {\color[HTML]{FE0000} 0.074345} \\
 & 135 & 1.2681 & 0.11211 & 0.11206 \\
 & 180 & 0.52274 & 0.17445 & 0.17449 \\
 & 225 & 0.42641 & 0.23627 & 0.23532 \\
 & 270 & 0.84819 & 0.2077 & 0.20105 \\
 & 315 & 0.70912 & 0.14262 & 0.13878 \\
\multirow{-8}{*}{10.5} & 360 & 0.25264 & 0.078113 & 0.077911 \\ \hline
\end{tabular}
\caption{Comparison between the optimal solution, the heuristic estimate and the multi-revolution Lambert for few test cases. Red values indicate an Hohmann transfer.}
\label{tab:comparison}
\end{table}

==> introduzioneOLD.tex <==

A multi-rendezvous (MRR) trajectory concerns the motion of an active spacecraft (chaser) which executes a sequence of maneuvers with the aim of performing a complete tour of a prescribed set of targets (e.g., space debris or asteroids).
MRR trajectories are gradually increasing in popularity within the aerospace community, as missions based on a chaser spacecraft ``hopping'' among multiple bodies are becoming of practical interest. Typical operational scenarios involve on-orbit servicing/refueling of geostationary satellites, and Active Debris Removal (ADR) missions.
ADR missions are particularly significant as they would allow to restore the functionality of the Low Earth Orbit (LEO) environment, close to being compromised by the huge amount of orbiting wreckage \cite{liou2008instability}. %Indeed, the LEO has already reached a critical state and its debris population will thus keep increasing even if no further launches will be made. 
Each ADR mission may involve the removal of several dozens of fragments, in order to reduce the cumulative cost of the operation. As a result, the best use of the  chaser propellant  becomes mandatory, and consequently, a well-designed trajectory must be searched for.

A number of authors dealt with long term or time-free ADR missions  aimed at removing a small number of debris from Sun synchronous orbits (at a rate of three to ten per year). 
These missions heavily rely on   $J_2$ orbital perturbation for the alignment of the orbital planes of consecutive targets before starting  the rendezvous maneuver, in order to reduce the mission cost.\cite{ shen2017optimization} 
 %\cite{braun2013active, cerf2013multiple, cerf2015multiple,
%
However, such an operational scenario becomes impractical in presence of strict time-constraints or long debris sequences. In this respect,
the present paper investigates the design of an ADR mission involving a tighter time-constraint and possibly longer target chains, assuming an impulsive thrust model for the chaser.
The aim is to minimize the overall mission $\Delta V$, while performing a complete tour of a prescribed set of targets that move on the same orbital plane at slightly different altitudes. 


The single-target time-fixed rendezvous is a well-known problem in spaceflight mechanics. Several optimization methods have been proposed assuming either finite \cite{Lu2012,Yue2009} or impulsive thrust \cite{Prussing1986, Mirfakhraie1994}.
In the latter case, four burns permit the achievement of the optimal solution, if close coplanar orbits are considered \cite{prussing1967optimal}.
Extension to a series of consecutive rendezvous is straightforward if the sequence of targets is assigned \textit{a priori} \cite{Jiang2016}.
However, the combinatorial aspect introduced by allowing permutations of the target sequence changes radically the problem nature and further increases its complexity. 
%
In this respect, the MRR problem presents several analogies with the Traveling Salesman Problem,\cite{lawler1985traveling} a well-known problem in Operational Research, where the goal is finding the shortest tour which allows a salesman to visit a prescribed set of cities. 

While similar, the problem here investigated is more complex than a standard TSP, as the cost associated with traveling between any two targets changes with time, due to the orbital motion. %, and \hl{for this reason}
%For this reason, the most effective tools, specifically developed for solving the TSP cannot be directly applied. 
%However, many buone cose non si possono usare
With this analogy in mind, 
several attempts have been made to find the optimal solution of the MRR problem by using algorithms developed in the context of %\hl{combinatorial optimization}
Operational Research.
%
Exhaustive, brute-force, approaches \cite{zuiani2012preliminary, braun2013active}  
and branch and bound search \cite{cerf2013multiple}
have been attempted first, for the design of optimal ADR missions in LEO.
However, the effectiveness of those methods is limited to small sets of targets, due to the \textit{course of dimensionality}.\cite{lenstra1981complexity} 
%deterministic approaches are viable only if small sets of targets are considered (with about ten elements or less). 
Meta-heuristic approaches have thus rapidly gained in popularity, as they allow to find a sub-optimal solution in a reasonable, limited amount of time.
%
Beam Search\cite{izzo2015evolving} and Ant Colony Optimization\cite{shen2017optimization}  have been widely exploited for both ADR 
and asteroid exploration mission planning. 
An hybridization of the two has also been discussed.\cite{simoes2017multi}
%
% stuart2016application
%
These methods attempt at chaining one target after the other, into a sequence,    
evaluating many (if not all)  possible branches departing from a given starting node.
In order to reduce the overall computational effort, 
simplistic transfer models are used for a fast evaluation of any target-to-target transfer cost;
moreover, pre-determined encounter epochs are commonly employed.\cite{zhang2018ant}
%
Despite being rather flexible, this formulation usually underperforms in case a complete tour is searched for. %, thus it might not be not appropriate for problem at hand.
Other methods, instead, rely on an iterative refinement of a set of (possibly random) initial solutions 
and guarantee the tour completeness at any point in the optimization process.
Prominent examples are Tabu Search (TS),\cite{gurtuna2003orbit} Simulated Annealing (SA),\cite{cerf2015multiple} and Genetic Algorithm (GA).\cite{liu2017multi,murakami2010approach, hokamoto2011genetic}
%all of which have been used on some specific problem instance/version.


%Motivation
Among the aforementioned optimization methods,
Genetic Algorithm is the most flexible one, as, in principle, it may handle any type of decision variable.
%Differently from tree-search methods as ACO o Beam Search,
GA performs a global optimization and, thanks to its stochastic selection and mutation operators,
it has greater chances to evade from local optima than greedy methods. In addition, it may adopt an encoding that guarantees the intrinsic completeness of the tour.
%
GA is a population-based method, hence
its execution time can be significantly reduced by an efficient parallel implementation, that is not possible for single-solution methods like TS and SA.
All these features make it a solid candidate for solving the complete tour problem here studied
and motivate its choice.

The paper is organized as follows.
Section~\ref{sez:statement} presents a comprehensive mathematical formulation of the impulsive multi-rendezvous problem, resulting in a Mixed-Integer Nonlinear Programming (MINLP) problem.
%
Section~\ref{sez:bilevelOpt} %tour
proposes a bi-level optimization approach aimed at solving it.
%
A simple heuristic is proposed in Section~\ref{sez:AnaliticalSolution}, based on a sub-optimal four-impulse analytic solution of the single-target rendezvous problem, for estimating the cost of each leg connecting two assigned consecutive targets once initial time and maximum transfer duration are prescribed.  The effectiveness of this sub-optimal solution is verified in a few relevant cases by comparing it with the optimal solution.
On the basis of this heuristic, a combinatorial optimization problem, or touring problem, is defined, which shares some features with the TSP. 
Section~\ref{sez:Tour} presents three formulations of the combinatorial problem with increasing complexity 
(which, in turn, provide increasing possibility of delivering the optimal solution of the original problem).
Section~\ref{sez:GA} describes the Generic Algorithm here adopted 
for the simultaneous optimization of the target sequence and rough estimation of the rendezvous epochs.
Once the best sequence and the approximate encounter times has been determined, the whole transfer is optimized through a multi-population self-adaptive Differential Evolution algorithm. Numerical results for a set comprising up to 15 targets are presented in Section~\ref{sez:results}.
A conclusion section ends the paper.

==> scarti.tex <==
cappello introduttivo sul TSP\\
-richiamo alle numerose formulazione ILP

Several formulations have been proposed with the aim of defining "stronger formulation",
that is, ...


\hl{formulazione }

\hl{l'idea e' presentare il tsp e formularlo direttamente nella forma permutazione
nel caso classico e nel caso TD-tsp TD2-TSP}



The classical TSP problem can be also formulated as an ordering problem.

let p be a permutation of $N_s$ elements,\\
pairwise cost c ij assegnati\\

se il costo dipende dalla posizione, 

$$
\sum_{i=1,N-1}{c_{\pi{i},\pi{i+1}}^{i}} + {c_{\pi{N},\pi{1}}^{N}} 
$$

passaggio al caso TD-TSP-2


formulazione del Time-Fixed Time-Discrete Tour

















%Picard and Queyranne [23] formulated the TDTSP over (V,A) as a linear
%integer program with the following set of constraints, where variable x t i,j with cost $c^t_{i,j} indicates if arc $(i,j,t)$$ is used and $N \ i denotes N \ {i}.









Nel caso del tsp classico, several formulations have been proposed

integer programming problem where
Arcs may be represented by binary variables, zero for no arc, one for an arc.




Presentare il problema tsp-td nelle varianti più generiche

ricordare che esistono diverse formulazioni

la maggior parte sono formulazioni Mixed-integer



presentare la formulazione mixed integer di Picard and Queyranne formulations
$$min_x \sum_{i,j,k}{c_{i,j}^k x_{i,j}^k}$$
$$ c1 $$
$$ c2 $$
$$ c3 $$
$$ c4 $$

Constraints c1-c4 serves to...


a number of constraints must be added in order to force








mostrare che la for












% IL TSP
The Traveling Salesman Problem (TSP) is a well-known combinatorial optimization problem, whose solution is the cheapest tour which allows a salesman to visit, only once, a number of cities in a map; the cost of each city-to-city transfer is, typically, the traveled distance or the fuel consumption. So, given a set of $N$ cities, with cost $c_{i,j}$ associated to the leg from city $i$ to $j$, the optimal tour is represented by the permutation $\pi$ of the numbers $\{1,\dots,N\}$ which minimizes $\sum_{i = 1}^{N - 1} c_{\pi(i), \pi(i+1)} $. 
In the time-dependent version of the problem (TDTSP), the cost associated with traveling  between any two cities changes with time. 
Among those present in literature, two TDTSP variants, with increasing complexity, are here considered: in approach (A), the cost $c_{i,j}$ to go from city $i$ to city $j$ is dependent only on the position of the leg $ij$ in the whole tour; in approach (B), the cost $c_{i,j}$ depends both on the starting time and on the duration of the transfer $ij$. 



The Time Dependent Traveling Salesman Problem (TDTSP) is a generalization of the classical Traveling Salesman Problem (TSP), where arc
costs depend on their position in the tour with respect to the source node.
While TSP instances with thousands of vertices can be solved routinely,
there are very challenging TDTSP instances with less than 100 vertices.













\hl{la formulazione deve matchare quella della sezione sopra}

-Time-Fixed Time-Uniform Tour

commentare dicendo che questa formulazione
permette di rappresentare 
tutti i casi descritti in precedenza

in particolare il TSP può essere vista come una istanza tempo-libero del problema
.. bla bla simmetria, etc

Il TSP-TD1 corrisponde al caso $D = 1$
mentre il caso TSP-TD2 al generico caso $N \times D$

